FedDebug: Systematic Debugging for Federated Learning Applications

In Federated Learning (FL), clients independently train local models and share them with a central aggregator to build a global model. Impermissibility to access clients' data and collaborative training make FL appealing for applications with data-privacy concerns, such as medical imaging. However, these FL characteristics pose unprecedented challenges for debugging. When a global model's performance deteriorates, identifying the responsible rounds and clients is a major pain point. Developers resort to trial-and-error debugging with subsets of clients, hoping to increase the global model's accuracy or let future FL rounds retune the model, which are time-consuming and costly. We design a systematic fault localization framework, FedDebug, that advances the FL debugging on two novel fronts. First, FedDebug enables interactive debugging of realtime collaborative training in FL by leveraging record and replay techniques to construct a simulation that mirrors live FL. FedDebug's breakpoint can help inspect an FL state (round, client, and global model) and move between rounds and clients' models seamlessly, enabling a fine-grained step-by-step inspection. Second, FedDebug automatically identifies the client(s) responsible for lowering the global model's performance without any testing data and labels--both are essential for existing debugging techniques. FedDebug's strengths come from adapting differential testing in conjunction with neuron activations to determine the client(s) deviating from normal behavior. FedDebug achieves 100% accuracy in finding a single faulty client and 90.3% accuracy in finding multiple faulty clients. FedDebug's interactive debugging incurs 1.2% overhead during training, while it localizes a faulty client in only 2.1% of a round's training time.

==> paper_sections/section_motivation.tex <==
% \section{Motivating Scenario}
% \label{motivating}

% This section presents a motivating example to demonstrate the debugging needs of FL applications. 
% Suppose that a machine learning application developer is given a task to train a model on federated learning for diagnosing different respiratory diseases (\eg Covid-19) from chest X-ray images of patients. Every participating hospital collects Chest X-rays of patients, which radiologists label, and then trains a local model on that data. The developer uses a convolutional neural network (CNN) such as ResNet \cite{he2015deep}. Hospitals periodically share their locally trained models with a central server, which are then aggregated into one global model using FedAvg~\cite{mcmahan2017communication}. The developer configures the FL server to request participating hospitals to send their locally trained model every 2 hours (round). 
% After aggregation, the central server sends the updated global model to each hospital to incorporate in local training in the next round. The FL architecture for this task is shown in Figure~\ref{fig:fl_base}.


% After a few days, one of the participating hospitals (say, Hospital A) notices a drop in the global model's accuracy on their local data. Deterioration in a model's performance in FL can arise due to a variety of reasons such as data corruption at a client or mislabelling by inexperienced and not well-equipped staff~\cite{chen2020focus}.

% \paragraph{Limitations for FL Debugging.} After noticing a drop in accuracy, the developer immediately starts investigating the root cause, as misdiagnosis can lead to unwanted delays and, in some cases,  life-threatening situations from ill-treatment. However, she faces challenges when debugging the FL application at this scale and finds manual inspection of collected logs to be her only option. She has access to the current global model, which she cannot evaluate due to inaccessibility to real-world test data in hospitals. The hospitals refrain from sharing their training process logging information as it might leak sensitive patient data. Hence, it is difficult to go back and forth across rounds to debug the FL application, reproduce the problem, and rectify the training from a disruptive round. Even if she can find the problematic round, she cannot isolate the hospital(s) responsible for affecting the accuracy, as statically inspecting hospitals' models does not reveal any information about the training data. Every hospital's model has different weights, even if they are equally accurate. Without any debugging techniques at her disposal, she has no choice but to either reset the global model or let the FL application continue, hoping that future rounds will help regain the lost accuracy.


% \paragraph{FedDebug for Interactive Debugging of FL Application.} The developer decides to use \tool to investigate the root cause of the issue, which she enables at the launch time of the FL application. 
% When a developer notices low model accuracy in her FL application, she sets a \tool's {\em breakpoint} at the end of the current round. 
% %
% FL application starts the aggregation step at the end of each round (\ie 2 hours)  which triggers \tool's breakpoint invoking a debugging session, a mirror of the original FL interface that is paused at the current round. 
% %
% In the debugging session, she uses \tool's step-back and step-next constructs to move between rounds, inspecting the global model and the hospitals' local model previously recorded by \tool. While it is discouraged to ask clients to evaluate the accuracy of the global model repetitively, \tool infrequently requests random clients to evaluate the global model's accuracy on their local data. 

% Upon inspecting the global model at different instances, she finds the specific round, {\tt R8},  where the performance starts to deteriorate. This round is different from the one reported by Hospital A as performance issues can manifest in earlier rounds but surface later. 
% %
% During this inspection, \tool also reports the list of hospitals that participated in that round. 
% Next, She invokes \tool's disruption client localization algorithm to identify the hospital responsible for disrupting the global model, leading to lower performance.  
% Lastly, after finding the disruptive client, the developer asks \tool to remove the disruptive hospital from the training from the problematic round, {\tt R8}, onwards. Its {\em fix and replay} performs retraining from round {\tt R8} to the current round, and then replaces the impacted global model with the retrained global model and continues the original Fl application. 
% %
% All of these steps require minimal effort from the developer. Without \tool, she will have to resort to using guesswork to identify the disruptive hospital or take no action. 








% \begin{comment}
% %With FedDebug, Alice can go back and forth to debug any round by utilizing the simulated breakpoint feature. To find out the abnormal clients while going back and forth, the FedDebug utilize FedFuzz approach. Since FedFuzz doesnt need any data to localize buggy clients, there will be zero privacy issues. After localizing the buggy clients, Alice will use Fix and Replay feature to fix the issue e.g., eliminate the bad performing clients or ask those hospitals to re-check their data and fix the issues like labelling etc. Now the traiing process will not resume from scratch but from that round. This will save subtantial time and resourse.   %Without \tool, she will have to use guesswork and inefficient statistical techniques. %
% %Since debugging session is a simulation of FL service, the developer cannot distinguish the simulation or real service and she can debug the service similar to debugging a live service. 
% %\gulzar{Need a diagram, similar to the limitation but this time we will show the benefits of \tool}%The possible solutions she send models to different clients to evaluate them which also leads to privacy issues. 

% \gulzar{Come up with a representative running example that should meet the following requirements: 1. Must help demonstrate each of the feature and the two FL setting (personalized and traditional). Explain the application first and then mention a case which requires debugging and currently very difficult for a user. Then list how FedDebug can solve each of those.} \waris{applied}

% % \waris{I am not sure how to include the Debug Construct 3 in this example.}
% % \waris{Labels in the real world are often noisy due to annotators’ varying skill-levels, biases or malicious tampering.}

% %Given the distributed training of FL, it is vulnerable to different errors such as noisy data and sign flipping attacks during the training process. Due to such issues, the clients become unreliable and hence result in lowering the performance of the global model. 



% %To find out the skewing clients, the Alice can use latency measuring feature to find out which clients are skewing the training process and then can remove such clients from the training, which might increase the performance of the global model.

% % Since in the existing FL libraries, there is no mechanism without accessing clients' data to find out the clients which are responsible for low performance of the global model. Without clients data access, it will be extremely challenging for FL engineer to localize such clients.



% %Alice starts the training from the central aggregator. The two possible scenarios in which she needs to debug the FL system are following:  i) global model's performance is deteriorating (e.g., model is misclassifying) due to lower resolution camera, faulty sensors, weather condition  ii) Model is not improving in its performance because there might be some training clients which are skewing the training process.


% %Consider a scenario where multiple hospitals from different cites collaborate to diagnose Covid-19 from chest X-rays. FL engineer deploys the model on each hospital (client). At the end of each day, the clients send their models to a central server for the aggregation. After the aggregation, the central server send model updates to each hospital. 


% % \gulzar{Next paragraph -- Problems. First problems is ..... second is .... third....}
% % After few days, one hospital realized that model is performing severely bad. The lower performing behavior can arise due to variety of reasons such data corruption, mislabelling, lack of expertise \& well-equipped staff.e.g., according to \cite{chen2020focus} the top tier hospitals are more reliable and make less mistakes in diagnosis as compared to low tier hospitals. Since in the existing FL libraries, there is no mechanism without accessing clients' data to find out the clients which are responsible for low performance of the global model. Without clients data access, it will be extremely challenging for FL engineer to localize such clients.    

% \gulzar{WE also need to focus on the compound impact of multiple low performance rounds. Becuase that will make it harder for the FL user to find from which round the problem started, which rounds were low performance, and what clients were involved. This will motivate the interactive debugging work because the user needs to inspect the rounds carefully to figure out what happened like going back and forth. } \waris{applied}


% \gulzar{ What is the current state of the art? instead we can focus on how user solve those issues today. here we say that the process is manual and mechanical, trial and error. There is a possibility of unreproducibility. so we need to attack the problem at runtime, right there and then. } \waris{applied}

% % With FedDebug, the user will not only be able to localize the problematic hospitals but can also identify when the behavior of these hospitals were shifting away from the normal behavior of other hospitals by utilizing the debugging construct 1 feature \textbf{step-in step-out} of the FedDebug. During the step-in, the user will use \textbf{differential execution and neuron coverage}  (Debugging Construct 2) to determine disruptive clients. Once the bad actors are identified, the user can apply fixes (Debugging Construct 3), e.g., eliminate the bad performing clients or ask those hospitals to re-check their data and fix the issues like labelling etc. After determining the disruptive clients and applying fixes, the user can start training from that specific point onwards instead of retraining from scratch to save time and resources. 
% %At launch time, the central server distributes the model's (\ie ResNet) weights and hyperparameters (\eg learning rate and regularization constant) among all the hospitals across the country. %Once the FL service is launched, each client starts collecting the training data locally ( X-rays images, in this case).  After a client collects adequate training data, it starts training the local model with global parameters and its own local data. 

% %, and in total of \todo{NN} times, also called rounds. commenting out this. round i 
% %We call an individual hospital \emph{client}.  Weights of a ResNet model include .... and they influence model's \gulzar{What are these weights and what are their impact}. %Similarly, the hyperparameters in ResNet include learning rate and regularization constant  and they direct influence the \gulzar{fill}. 



% %The developer sets the total number of rounds to be NN where each round is YY hours long. With this setting, the FL server will ask all  participating clients to send their locally trained model every yy hours, and in total of NN times. At the end of each round, all participating clients send their local trained weights to the central server for aggregation. In this setting, the developer has configured the IBMFL framework to use {\tt FedAvg}\cite{mcmahan2017communication}, which is analogous to vector-based average operation. 
% %The central server performs the aggregation of these weights by using an aggregator algorithm such as FedAvg . 
% %At the end of each day, the clients send their models to a central server for the aggregation i.e., one training round per day. 
% %document that low-ranked hospitals are more likely to mislabel medical imaging data. 

% %\gulzar{For limitations: We need one figure showing all the issues. }





% % \subsection{Autonomous Vehicle Example}
        
    
%     % Suppose that Alice is an ML engineer who is given the task to develop a FL solution for autonomous vehicles (AVs) to detect \& classify objects such cars, trucks, bicycles, pedestrians, barrier, traffic cones etc. Such tasks are very critical for the safety of AVs. The FL architecture for this task is shown in Figure [add figure]. Alice uses a convolutional neural network (CNN) such as  ResNet \cite{he2015deep} for this task and video feed from AVs cameras. Initially, the global server distribute ResNet weights and hyperparameters (e.g., learning rate, regularization constant etc.) among all the clients which in this case are vehicles. After parameters sharing, each client train its local model with these parameters and on its own local data. At the end of each round, clients share the local trained weights with the global server for the aggregation. The central server performs the aggregation of these weights by using an aggregator algorithm such as FedAvg \cite{mcmahan2017communication}. Each round is performed after 30 minutes and Alice selects  clients based on their availability, e.g., connected to a power supply and have stable internet connection.
%     % Alice starts the training from the central aggregator. The two possible scenarios in which she needs to debug the FL system are following:  i) global model's performance is deteriorating (e.g., model is misclassifying) due to lower resolution camera, faulty sensors, weather condition  ii) Model is not improving in its performance because there might be some training clients which are skewing the training process.   
    
%     % \textbf{Limitations for FL Debugging.} To debug the above problems, Alice will face several limitations with the traditional approaches. First, it's extremely challenging for Alice to determine the problematic round. Second, it's quite difficult to evaluate models. Third clients might not be logging information related to each round, which make it also difficult to go back and forth to debug FL system, recreate the problem, and restart training from a buggy round. Even Alice ask clients to log such information, she doesn't have any technique in her tool box to localize the buggy clients without accessing the clients' data. The possible solutions she might have is to access the clients data to evaluate model which violates FL properties or send models to different clients to evaluate them which also leads to privacy issues. 
    
%     % \textbf{FedDebug for Interactive Debugging of FL System.} With FedDebug, Alice can go back and forth to debug any round by utilizing the simulated breakpoint feature. To find out the abnormal clients while going back and forth, the FedDebug utilize differential testing feature. Since no data is needed, there will be zero privacy issues. After localizing the buggy clients, Alice will use Fix and Replay feature by removing such clients models in the aggregations and resume training from that points onwards and hence not require restarting training from the scratch. To find out the skewing clients, the Alice can use latency measuring feature to find out which clients are skewing the training process and then can remove such clients from the training, which might increase the performance of the global model.    
%     \waris{Issue: FedML itself is for entripise and latency monitiong feature is very common ..  we can skip it . }

% \end{comment}




==> tables/global_acc.tex <==
\begin{tabular}{rrr}
\toprule
 Num of Flip Labels &  Global Model Prediction Accuracy (CIFAR-10) &  Global Model Prediction Accuracy (FEMNIST) \\
\midrule
                  0 &                                         0.74 &                                        0.66 \\
                  2 &                                         0.73 &                                        0.63 \\
                  3 &                                         0.72 &                                        0.61 \\
                  4 &                                         0.71 &                                        0.64 \\
                  5 &                                         0.71 &                                        0.62 \\
                  6 &                                         0.72 &                                        0.55 \\
                  7 &                                         0.69 &                                        0.60 \\
                  8 &                                         0.66 &                                        0.52 \\
                  9 &                                         0.58 &                                        0.56 \\
\bottomrule
\end{tabular}


==> tables/table-model-params.tex <==
\begin{tabular}{| r | r | r | r |}
\toprule
{\bf ResNet-18} & {\bf ResNet-50} & {\bf DenseNet-121} & {\bf VGG-16} \\
\midrule
 11.2 M &     23.5 M &        7 M  &      134 M \\
\bottomrule
\end{tabular}


==> tables/table_flip_2_9.tex <==
\begin{tabular}{rrrrr}
\toprule
 Flipped Labels &  Avg. Accuracy (ResNet-34) &  Avg. Accuracy (DenseNet-121) &  Avg. Detection Time (s) &  Avg. Input Time (s) \\
\midrule
               2 &                      10.00 &                          1.00 &                     0.15 &                 2.40 \\
               3 &                      32.00 &                         50.00 &                     0.15 &                 2.40 \\
               4 &                      87.50 &                         58.00 &                     0.17 &                 2.40 \\
               5 &                      50.00 &                         50.00 &                     0.17 &                 2.40 \\
               6 &                      50.00 &                         99.00 &                     0.17 &                 2.40 \\
               7 &                     100.00 &                         53.00 &                     0.15 &                 2.40 \\
               8 &                     100.00 &                         99.50 &                     0.15 &                 2.40 \\
               9 &                     100.00 &                        100.00 &                     0.25 &                 2.40 \\
\bottomrule
\end{tabular}

